Characterization theorems for PDL and FO(TC)

Our main contributions can be divided in three parts: (1) Fixpoint extensions of first-order logic: we give a precise syntactic and semantic characterization of the relationship between $\mathrm{FO(TC^1)}$ and $\mathrm{FO(LFP)}$; (2) Automata and expressiveness on trees: we introduce a new class of parity automata which, on trees, captures the expressive power of $\mathrm{FO(TC^1)}$ and WCL (weak chain logic). The latter logic is a variant of MSO which quantifies over finite chains; and (3) Expressiveness modulo bisimilarity: we show that PDL is expressively equivalent to the bisimulation-invariant fragment of both $\mathrm{FO(TC^1)}$ and WCL. In particular, point (3) closes the open problems of the bisimulation-invariant characterizations of PDL, $\mathrm{FO(TC^1)}$ and WCL all at once.

==> extra.tex <==
% !TEX root = main.tex

%%%%
\section*{Extra: Logical characterization of $\AutWA(\ofoe)$ on all models}
\textbf{This could be done.}

Graded PDL. 
\begin{align*}
    \varphi &::= p \mid \lnot \varphi \mid \varphi \lor \varphi
        \mid \tup{d}_{\geq k} \mid \tup{\prog}\varphi \\
    \prog &::= d \mid \prog\seq\prog \mid \prog\choice\prog \mid \prog^\star 
        \mid \varphi?
\end{align*}
\fcerror{cite, janin}Cite the original result saying that $\Aut(\ofoe) \equiv \muML_{\geq}$.

\begin{theorem}
	$\AutWA(\ofoe) \equiv \pdl_\geq$ on all models.
\end{theorem}

The key observations are: (1) this
\[
\dbnfofoe{\vlist{T}}{\Pi} = \exists \vlist{x}.\big(\arediff{\vlist{x}} \land \bigwedge_i \tau_{T_i}(x_i) \land \forall z.(\arediff{\vlist{x},z} \lthen \bigvee_{S\in \Pi} \tau_S(z))\big)
\]
(recall that $\Pi\subseteq\vlist{T}$) can be translated as
\[
\Box \bigvee\vlist{T} \land \bigwedge_{T_i\in\vlist{T}} exact(T_i)
\]
where $exact(T_i) = \Diamond_k T_i \land \lnot \Diamond_{k+1} T_i$ and $k=\sharp{T_i} \in \vlist{T}$.

and (2): because of complete additivity variables bound by fixpoints ``cannot appear'' under a graded modality (i.e., in the automata, think of cycles)

This corollary should be interesting for databases.
\begin{corollary}
	$\binfotc \equiv \pdl_{\geq}$ over tree models.
\end{corollary}

Also in Description Logics: $\mathcal{ALC}_\text{reg}$ is PDL~\cite{Schild91acorrespondence}. And $\mathcal{ALCQ}_\text{reg}$ seems to be exactly the kind of graded PDL I want~\cite{DBLP:journals/corr/abs-1104-1964} (check).

%%%%
\section*{Extra: Bisimulation quantifiers for \pdl}
\textbf{This could be done.}

We define some bisimulation quantifiers:
\begin{align*}
\model,s \mmodels \bq p.\varphi & \quad\text{ iff }\quad \model'[p\mapsto X_p],s' \mmodels \varphi \text{ for some arbitrary $X_p\subseteq \moddom$}\\
\model,s \mmodels \wcbq p.\varphi & \quad\text{ iff }\quad \tmodel[p\mapsto X_p],s \mmodels \varphi \text{ for some finite chain $X_p\subseteq \tmoddom$}
\end{align*}
where $(\model',s')$ is some model bisimilar to $(\model,s)$ and $(\tmodel,s)$ is a \emph{tree} bisimilar to $(\model,s)$.

\begin{proposition}
	$\pdl$ is closed under $\wcbq$.
\end{proposition}
\begin{proof}
	\fcerror{Do}Look at $\alpha\in\pdl$ as an automaton $\aut\in\AutWA(\ofoe)$. Use closure of $\AutWA(\ofoe)$ under projection (on trees!) together with some unravelling tricks and that $\AutWA(\ofoe)$ are invariant under counting bisimulation (and that a normal unravelling is counting bisimilar to the original model).

	Maybe just use translation to \wcl and $(-)^\bullet$.
\end{proof}

\begin{remark}
	Actually we could have defined the quantifier as
	\[
	\model,s \mmodels \wcbq p.\varphi \quad\text{ iff }\quad \model'[p\mapsto X_p],s' \mmodels \varphi \text{ for some finite chain $X_p\subseteq \moddom$}
	\]
	where $(\model',s')$ is some model bisimilar to $(\model,s)$ with the crucial condition that there is no element $t$ colored with $p$ such that $R^+(t,t)$. The idea is that we don't want the automaton to be able to use a finite chain to read infinitely many $p$'s. A slightly modified proof of the above proposition goes through.

	This remark also means that the closure also restricts to finite models (via partial unravellings).
\end{remark}

\begin{theorem}
	$\pdl \equiv \ML(\Box^*,\wcbq)$.
\end{theorem}
\begin{proof}
	\fcerror{Do}The $\supseteq$ inclusion is by the above proposition. For the other direction we consider \pdl as $\mucaML$ and show that we can encode completely additive fixpoint using $\Box^*$ and $\wcbq$.
\end{proof}


==> soaut-fixpoint.tex <==
% !TEX root = main.tex

REMOVE

\begin{definition}
Let $\aut = \tup{A, \tmap, \pmap, a_I}$ be an additive-weak automaton on alphabet $\pw(\oprops \dcup \{p\})$.
We define the \emph{iteration of $\aut$ over $p$} as the automaton ${\mu p}.\aut := \tup{A^{\mu},
\tmap^{\mu}, \pmap^{\mu}, a_I^{\mu}}$ on alphabet $\wp(\oprops)$ by putting
%
\[
\tmap^\mu(a,c) := \tmap(a,c) \lor \big(\tmap(a,c\cup\{p\}) \land \tmap(a_I,c\cup\{p\})\big)
\]
%
\fcerror{check}for every $c\in \wp(\oprops)$.
\end{definition}

\begin{definition} Let $p\notin\oprops$ and $L$ a tree language of $\pw(\oprops\dcup\{p\})$-labeled trees. The \emph{iteration} of $L$ over $p$ is the language $\mu p.L$ of $\pw(\oprops)$-labeled trees defined as
\[
  \mu p.L := \{\model \mid \model[p\mapsto S] \in L \text{ for ... } \}.
\]
\end{definition}


